Quadratic differentials as stability conditions: collapsing subsurfaces

We introduce a new class of triangulated categories, which are Verdier quotients of three-Calabi-Yau categories from (decorated) marked surfaces, and show that its spaces of stability conditions can be identified with moduli spaces of framed quadratic differentials on Riemann surfaces with arbitrary order zeros and arbitrary higher order poles. A main tool in our proof is a comparison of two exchange graphs, obtained by tilting hearts in the quotient categories and by flipping mixed angulations associated with the quadratic differentials.

==> packages.tex <==

%languages, pictures
\ProvidesPackage{language}
\usepackage{lmodern}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
%\usepackage{csquotes}
\usepackage{graphicx,color}
\usepackage[colorlinks, linkcolor=blue!50,anchorcolor=Periwinkle,
citecolor=blue!72,urlcolor=cyan, bookmarksopen,bookmarksdepth=2]{hyperref}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{anyfontsize}
\usepackage{comment}

%biblatex
%\usepackage[style=alphabetic,backend=bibtex,maxnames=10]{biblatex}
\usepackage[style=alphabetic,
            isbn=false,
            doi=false,
            url=false,
            backend=bibtex,
            maxnames=5,
            maxalphanames=5,firstinits=true
           ]{biblatex}
%\usepackage{layout}
\usepackage{enumitem}
\usepackage{afterpage}
%\usepackage{parskip}
\usepackage{aliascnt}
%\usepackage[notref,notcite]{showkeys}
\usepackage{xparse}
\usepackage{caption}
%\usepackage{tabto}
\usepackage{imakeidx}
%\usepackage[normalem]{ulem}
\allowdisplaybreaks


%math
\usepackage{amsmath,amsfonts,amsthm,mathtools,amssymb}
\usepackage{tensor}
\usepackage{amscd,latexsym, mathrsfs, epsfig}
\usepackage{mathdots}
\usepackage{upgreek}
%\usepackage{enumerate}
%\usepackage{undertilde}
\usepackage[all]{xy}
\usepackage{transparent}
%tikz
\usepackage{tikz}
\usepackage{tikz-cd}
\usepackage{float}
\usepackage{circuitikz}
\usetikzlibrary{positioning}
\usetikzlibrary{matrix, calc, arrows, decorations.pathreplacing, decorations.markings, decorations.pathmorphing, backgrounds,fit,positioning,shapes.symbols,chains,shadings,fadings}
\usetikzlibrary{cd}
\usetikzlibrary{intersections}
\tikzset{
	every loop/.style={very thick},
	comp/.style={circle,black,draw,thin,inner sep=0pt,minimum size=5pt,font=\tiny},
	order bottom left/.style={pos=.05,left,font=\tiny},
	order top left/.style={pos=.9,left,font=\tiny},
	order bottom right/.style={pos=.05,right,font=\tiny},
	order top right/.style={pos=.9,right,font=\tiny},
	%
	order middle right/.style={draw,thin,shape=rectangle,inner sep=2pt,outer sep=5pt,pos=.5,right,font=\tiny},
	%
	order middle left/.style={draw,thin,shape=rectangle,inner sep=2pt,outer sep=5pt,pos=.5,left,font=\tiny},
	%	
	order node dis/.style={text width=.75cm},
	circled number/.style={circle, draw, inner sep=0pt, minimum size=12pt},
	below left with distance/.style={below left,text height=10pt},
	below right with distance/.style={below right,text height=10pt}
}

\tikzset{->-/.style={decoration={  markings,  mark=at position #1 with
			{\arrow{>}}},postaction={decorate}}}
\tikzset{-<-/.style={decoration={  markings,  mark=at position #1 with
			{\arrow{<}}},postaction={decorate}}}

